Stochastic Mirror Descent for Large-Scale Sparse Recovery

In this paper we discuss an application of Stochastic Approximation to statistical estimation of high-dimensional sparse parameters. The proposed solution reduces to resolving a penalized stochastic optimization problem on each stage of a multistage algorithm; each problem being solved to a prescribed accuracy by the non-Euclidean Composite Stochastic Mirror Descent (CSMD) algorithm. Assuming that the problem objective is smooth and quadratically minorated and stochastic perturbations are sub-Gaussian, our analysis prescribes the method parameters which ensure fast convergence of the estimation error (the radius of a confidence ball of a given norm around the approximate solution). This convergence is linear during the first "preliminary" phase of the routine and is sublinear during the second "asymptotic" phase. We consider an application of the proposed approach to sparse Generalized Linear Regression problem. In this setting, we show that the proposed algorithm attains the optimal convergence of the estimation error under weak assumptions on the regressor distribution. We also present a numerical study illustrating the performance of the algorithm on high-dimensional simulation data.

==> uniform_convexity_analysis.tex <==
\section{Analysis with uniform convexity hypothesis around the optimum}

\textcolor{blue}{
In this section we are going to derive the same analysis but in a much more complex setting. Here we will consider that the objective function $g$ is lower bounded as follows
\[
g(x) - g(x_*) \geq \mu\left(\|x-x_*\|_{\Sigma}\right).
\]
Where $\mu (x) = \frac{\mu}{p} |x|^p$ such that its Legendre-Fenchel transform is $\mu^*(y) = \frac{\mu^{1-q}}{q} |y|^q$ with $ \frac{1}{p}+\frac{1}{q} = 1$. Similar to the analysis given in Subsection \ref{sec:multi_alg}, we introduce the {\em Reduced Uniform Convexity} assumption.
\paragraph{Assumption [RUC]}
There exist some $\psi>0$  and $\rho<\infty$ such that for any feasible solution $\widehat{x} \in X$ to the composite problem \rf{eq:comp} satisfying, with probability at least $1-\varepsilon$,
\[
    F_{\kappa}(\widehat{x}) - F_\kappa(x_*) \leq \upsilon,
\]
it holds, with probability at least $1-\varepsilon$, that % given monotone nondecreasing function $\varrho:\,\bR_+\to \bR_+$, and $\theta>0$,
%\be
%    \Prob\left\{\|\wh x - x_*\|\leq \theta\kappa^{-1}\left[\varrho\left(\kappa\sqrt{s}\right) + \upsilon\right]\right\}\geq 1-\epsilon.
%\ee{eq:lem}
%In particular, in the case of quadratic $\varrho(t)={\rho\over 2} t^2$, in which case  the bound \rf{eq:lem} reads
\be
\|\wh x - x_*\|\leq \frac{1}{\psi \kappa}\left[\rho s^{\frac{q}{2}}\kappa^q + {\upsilon}\right].
\ee{eq:lemunif}
}





Recall that by Lemma \ref{lemm1} we have 
\[
\psi^{-1}\|x-x_*\| \leq {\kappa}^{-1}\left({\mu^*(\kappa\sqrt{\sfrac{s}{\lambda}})} + {\upsilon}\right),
\]
where $\upsilon$ is either bound \eqref{eq:almo} or \eqref{eq:almo2} on the deviation of the penalized objective function $F_{\kappa}$, depending whether we are in the minibatch setting or not.
The uniform convexity setting is obtained when choosing $\mu(x) = \mu |x|^{\beta}$, where $\mu$ is the constant of uniform convexity, this mapping has for Legendre-Fenchel conjugate the function $\mu^*(y) = (\beta-1)\left|\frac{y}{\beta\mu^{1\over\beta}}\right|^{\beta\over{\beta-1}}$, for the rest of the study we assume $\beta > 2$.\\
In what follows, we present the results for the minibatch setting. Note that with a similar analysis as what is exposed in Subsection \ref{sec:multi_alg}, it is possible to derive similar results for the vanilla CSMD setting.

\begin{lemma}
 \label{lem:unifconv}
Let $k$ denote the number of the current stage in the preliminary phase. We choose $m^{(p)}_k \asymp \psi^{\beta} R_{k-1}^{2 - \beta } \mu^{-1} \sqrt{\sfrac{s}{\lambda}}^{\beta} \left(\Theta + t \right)$, $\gamma = (4\nu)^{-1}$, and let $t$ satisfy $t\geq 4\sqrt{2+\log(m^{(p)}_{\ov K_1})}$.
\par
Suppose that $R \gtrsim \frac{\sigma_*^{\frac{2}{\beta}} \psi \sqrt{\sfrac{s}{\lambda}}}{(\nu \mu)^{\frac{1}{\beta}}}$ , that initial condition $x_0$ of Algorithms \ref{alg2} and \ref{alg3} satisfies $\|x_0-x_*\|\leq R$, and that at the stage $k$ of the preliminary phase we choose
\be\kappa_k \asymp \frac{R_{k-1}^{\beta - 1} \mu }{\psi^{\beta - 1} \sqrt{\sfrac{s}{\lambda}}^{\beta}}
\ee{kappa_k} where  $(R_k)_{k\geq 0}$ is defined recursively:
\[
R_{k+1} = \frac{R_{k}}{2} +  \frac{\sigma_*^2 \left(\psi \sqrt{\sfrac{s}{\lambda}}\right)^{\beta}}{\beta \mu \nu R_{k}^{\beta - 1}}2^{\left(2 + \frac{1}{\beta}\right)(\beta-1) + 1} ,\quad R_0=R.
\]
Then the approximate solution $\wh x_{m^{(p)}_k}^k$ at the end of the $k$th stage of the CSMD-SR algorithm satisfies, with probability at least $ 1-4ke^{-t}$
\be
    \|\wh{x}_{m^{(p)}_k}^k-x_*\| &\leq R_k  \leq 2^{-k}R +  \frac{3\sigma_*^{\frac{2}{\beta}}\psi \sqrt{\sfrac{s}{\lambda}}}{(\beta - 1)(\mu \nu)^{\frac{1}{\beta}}}2^{\beta + 1},
    %\\&\leq R_0\exp\left(-\frac{M_k}{32\psi^2 \rho s \nu(4\Theta +39t)}\right) + 2\sigma_*\psi\sqrt{6\rho s\nu^{-1}}.
\ee{ya2uc}
In particular, the estimate $\wh{x}^{\ov{K}_1}_{m^{(p)}_{\overline{K}_1}}$ after $\overline{K}_1 \asymp \log_2\left(\frac{R^{\beta}\nu \mu}{ \sigma^2_* \psi^{\beta}(\sqrt{s/\lambda})^{\beta}}\right) $ stages  satisfies with probability at least $1-4\ov{K}_1 e^{-t}$
\be\|\wh{x}_{m^{(p)}_{\overline{K}_1}}^{\overline{K}_1}-x_*\|\lesssim \psi\sqrt{\sfrac{s}{\lambda}}\left({\sigma_*^2\over\nu\mu}\right)^{1\over\beta}.
\ee{prelim-phaseuc}
\end{lemma}

\paragraph{Proof.}
First let us observe that under the hypothesis validating Proposition \ref{pr:mupropn}, we have with probability at least $1-4e^{-t}$ that, for $\wh x_m$ an approximate solution obtained after having applied $m$-step of the CSMD algorithm, the following inequalities hold true
\begin{align*}
     {F}(\wh x_m) - {F}(x_*)
    &\leq  \frac{R^2}{m \gamma}(\Theta + 15t) + \frac{\kappa R}{m} + \sigma^2_*\gamma\left(7 + \frac{24t}{m}\right) := \upsilon\nonumber
\end{align*}
Recall that with the choice $\gamma = \frac{1}{4\nu}$, $\upsilon$ becomes 
\[
\upsilon = \frac{R^2\nu}{m}(4\Theta + 60t) + \frac{\kappa R}{m} + \frac{\sigma_*^2}{\nu}\left(\frac{7}{4}+\frac{6 t}{m}\right).
\]
Let now apply Lemma \ref{lemm1} in the exact $s$-sparsity assumption within the uniform convexity framework, we then have 
\begin{align}
\|\wh x_m - x_*\| \leq \psi \left[(\beta -1) \left(\frac{\sqrt{\sfrac{s}{\lambda}}}{\beta \mu^{\frac{1}{\beta}}}\right)^{\frac{\beta}{\beta -1}}\kappa^{\frac{1}{\beta - 1}}+\frac{\nu R^2}{m \kappa}\left(4\Theta + 60t\right) +\frac{R}{m} + \frac{\sigma_*^2}{\kappa \nu}\left(\frac{7}{4} + \frac{6t}{m}\right) \right].\label{prooflemm4.1-1}
\end{align}
The rest of the proof is carried by induction, it consists in applying result \eqref{prooflemm4.1-1} for each stage of the algorithm and choosing its parameters accordingly to the statement of Lemma \ref{lem:unifconv}. \\

{\bf 1$^o$.} Note that initial point $x_0$ satisfies $x_0\in X_R(x_*)$. Suppose that the initial point $x^k_0=\wh x^{k-1}_{m_{k-1}}$ of the $k$th stage of the method satisfy $x_0^k\in X_{R_{k-1}}(x_*)$ with probability $1-4(k-1)e^{-t}$. 
In other words, there is a set $\B_{k-1}\subset \Omega$, with $\Prob(\B_{k-1})\geq 1-4(k-1)e^{-t}$, such that for all $\ov\omega^{k-1}=[\omega_1;...;\omega_{m_{k-1}(k-1)}]\subset \B_{k-1}$ one has $x_0^k\in X_{R_{k-1}}(x_*)$. 
Let us show that upon termination of the $k$th stage $\wh x^k_{m_k}$ satisfy $\|\wh x_{m_k}^k-x_*\|\leq R_k$ with probability  $1-4ke^{-t}$.
By result \eqref{prooflemm4.1-1}
we conclude that for some $\ov\Omega_k\subset \Omega$, $\Prob(\ov\Omega_k)\geq 1-4e^{-t}$, solution $\wh{x}^k_{m_0}$  after $m_0$ iterations of the stage satisfies, for all 
for all $\omega^k=[\omega_{(k-1)m_{k-1}+1},...,\omega_{km_k}]\in \ov\Omega_k$,
\begin{align}
\|\wh x^k_{m_{k}} - x_*\| \leq \psi \left[(\beta -1) \left(\frac{\sqrt{\sfrac{s}{\lambda}}}{\beta \mu^{\frac{1}{\beta}}}\right)^{\frac{\beta}{\beta -1}}\kappa_{k}^{\frac{1}{\beta - 1}}+\frac{\nu R_{k-1}^2}{m_k \kappa_k}\left(4\Theta + 60t\right) +\frac{R_{k-1}}{m_k} + \frac{\sigma_*^2}{\kappa_k \nu}\left(\frac{7}{4} + \frac{6t}{m_k}\right) \right].\label{prooflemm4.1-2}
\end{align}
We now choose $\kappa_k$ in order to minimize the first two terms of equation \eqref{prooflemm4.1-2}, i.e., 
\[
\kappa_k = \beta \mu^{\frac{1}{\beta}}\sqrt{\sfrac{\lambda}{s}} \left(\frac{\nu R_{k-1}^2(4\Theta + 60t)}{m_k}\right)^{1 - \frac{1}{\beta}}
\]
Plugging this into \eqref{prooflemm4.1-2} gives
\begin{align}
\|\wh x^k_{m_{k}} - x_*\| \leq \psi \left[\sqrt{\sfrac{s}{\lambda}}\left(\frac{\nu (4\Theta + 60t)}{m_k \mu}\right)^{\frac{1}{\beta}}R_{k-1}^{\frac{2}{\beta}} +\frac{R_{k-1}}{m_k} + \frac{\sigma_*^2}{\beta \mu^{\frac{1}{\beta}} \nu \sqrt{\sfrac{\lambda}{s}}}\left(\frac{7}{4} + \frac{6t}{m_k}\right) \left(\frac{m_k}{\nu R_{k-1}^2(4\Theta + 60t)}\right)^{1 - \frac{1}{\beta}}\right].\label{prooflemm4.1-3}
\end{align}
Now observe that by choosing the length of each stage such that 
\[
m_k =  \left\lceil 4^{\beta}\psi^{\beta}\sqrt{\sfrac{s}{\lambda}}^{\beta}\nu\mu^{-1}(4\Theta + 60t) R_{k-1}^{2-\beta}\right\rceil, 
\] 
we have that each of the first two terms of \eqref{prooflemm4.1-3} is bounded by $\frac{R_{k-1}}{4}$. Furthermore, observe that when choosing $m_k$ as shown above, we have that $m_k \leq 2\psi^{\beta}\sqrt{\sfrac{s}{\lambda}}^{\beta}\nu\mu^{-1}(4\Theta + 60t) R_{k-1}^{2-\beta}$ and $\frac{6t}{m_k} \leq \frac{1}{4}$. Altogether, this results in 
\begin{align}
\|\wh x^k_{m_{k}} - x_*\| \leq \frac{R_{k-1}}{2} +  \frac{\sigma_*^2 \left(\psi \sqrt{\sfrac{s}{\lambda}}\right)^{\beta}}{\beta \mu \nu R_{k-1}^{\beta - 1}}2^{\left(2 + \frac{1}{\beta}\right)(\beta-1) + 1} = R_k.\label{prooflemm4.1-4}
\end{align}
We conclude that $\wh{x}^k_{m_0}\in X_{R_k}(x_*)$ for all $\ov\omega^k\in \B_k=\B_{k-1}\cap \ov\Omega_k$, and \[\Prob(\B_k)\geq \Prob(\B_{k-1})-\Prob(\ov\Omega_k^c)\geq 1-4ke^{-t}.\]\\
{\bf 2$^o$.}
Let now $a=\frac{\sigma_*^2 \left(\psi \sqrt{\sfrac{s}{\lambda}}\right)^{\beta}}{\beta \mu \nu }2^{\left(2 + \frac{1}{\beta}\right)(\beta-1) + 1}$, and let us study the behaviour of the sequence
\begin{align*}
R_{k} = \frac{R_{k-1}}{2} +\frac{a}{R_{k-1}^{\beta - 1}}=:f(R_{k-1}), \quad R_0=R \geq \frac{\left(2a\right)^{\frac{1}{\beta}}\beta}{2(\beta - 1)^{\frac{\beta - 1}{\beta}}}. 
\end{align*}
Function $f$ admits a minimum at $R= \left(2(\beta - 1)a\right)^{\frac{1}{\beta}}$ and its minimum is $  \frac{\left(2a\right)^{\frac{1}{\beta}}\beta}{2(\beta - 1)^{\frac{\beta - 1}{\beta}}}$, so one has  $R_k\geq \frac{\left(2a\right)^{\frac{1}{\beta}}\beta}{2(\beta - 1)^{\frac{\beta - 1}{\beta}}}$, $\forall k$. Thus, by using this result, we can upper bound $R_{k-1}^{-(\beta-1)}$ as follows, $R_{k-1}^{-(\beta-1)}\leq \frac{2^{\beta-1}(\beta - 1)^{\frac{(\beta - 1)^2}{\beta}}}{\left(2a\right)^{\frac{\beta - 1}{\beta}}\beta^{\beta-1}}$. This, together with \eqref{prooflemm4.1-4} results in
\[
\|\wh x^{k}_{m_k} - x_*\| \leq \frac{1}{2}R_{k-1} + \frac{\sigma_*^{\frac{2}{\beta}}\psi \sqrt{\sfrac{s}{\lambda}}}{(\mu \nu)^{\frac{1}{\beta}}} \underbrace{\frac{2^{\beta +\frac{2}{\beta} + (2 + \frac{1}{\beta})\frac{(\beta - 1)}{\beta} } (\beta - 1)^{\frac{(\beta - 1)^2}{\beta}}}{\beta^{\beta - 1 +\frac{1}{\beta}}}}_{= \alpha}
\]
Note that with simple calculations, one can show that, $\forall \beta\geq 2$, 
\[
\frac{(\beta-1)^{\frac{(\beta-1)^2}{\beta}}}{\beta^{\beta-1+\tfrac{1}{\beta}}} \leq \frac{e^{e^{-1}-1}}{\beta-1}, \quad \text{and} \quad 2^{\beta +\frac{2}{\beta} + (2 + \frac{1}{\beta})\frac{(\beta - 1)}{\beta} } \leq 2^{\beta + \frac{9}{4}}
\]
this gives that,
\[
\alpha \leq 3\frac{ 2^{\beta}}{\beta - 1}.
\]
We can then prove, by using the recursive relationship among the elements of the sequence $(R_k)_{k\geq0}$ that
\begin{align*}
    \|\wh x^{k}_{m_k} - x_*\| \leq 2^{-k}R +  \frac{3\sigma_*^{\frac{2}{\beta}}\psi \sqrt{\sfrac{s}{\lambda}}}{(\beta - 1)(\mu \nu)^{\frac{1}{\beta}}}2^{\beta + 1},
\end{align*}
which is \rf{ya2uc}.
Finally, 
after running $\overline{K}_1 = \left\lceil\frac{1}{\beta}\log_2\left(\frac{R^{\beta}(\beta -1)^{\beta}\mu \nu}{3^{\beta} \sigma^2_* \psi^{\beta}(\sqrt{\sfrac{s}{\lambda}})^{\beta}2^{\beta(\beta + 1)}}\right)\right\rceil$ stages of the preliminary phase, the estimate $\wh{x}^{\overline{K}_1}_{m_0}$ satisfies
\begin{align*}
    \|\wh x^{\ov K_1}_{m_{\ov K_1}} - x_*\| \leq \frac{3\sigma_*^{\frac{2}{\beta}}\psi \sqrt{\sfrac{s}{\lambda}}}{(\beta - 1)(\mu \nu)^{\frac{1}{\beta}}}2^{\beta + 2}.
\end{align*}

This finally, concludes the proof of the lemma.
\qed

We can now move on to the results regarding the second phase of the algorithm.

\begin{lemma}
\label{lem:unifconv2}
%\textbf{Second "Asymptotic" phase (mini-batch setting):}
Let $k$ denote the number of the current stage in the asymptotic phase. Take $\gamma=(4\nu)^{-1}$, $\ell_k \asymp 2^{k\beta}\chi \Theta $, $\kappa_k \asymp 2^{-k(\beta-1)}\mu^{1\over\beta}\sqrt{\sfrac{\lambda}{s}}\left(\frac{  \sigma_*^2}{\nu}\right)^{\frac{\beta -1}{\beta}}$ with $m^{(a)}_k \asymp 2^{(\beta - 2)k}(\Theta + t) \mu^{-\frac{2}{\beta}}\nu^{\frac{2(\beta - 1)}{\beta}} \psi^{2}s{\lambda^{-1}}\sigma_*^{\frac{2(2-\beta)}{\beta}} $,
\[r_k=2^{-k}r_0, \quad \text{and} ,\quad r_0=\frac{3\sigma_*^{\frac{2}{\beta}}\psi \sqrt{\sfrac{s}{\lambda}}}{(\beta - 1)(\mu \nu)^{\frac{1}{\beta}}}2^{\beta + 2}.%10\frac{2^{-k}\psi\sigma_*}{\sqrt{ N_2}}\sqrt{2(\Theta+\tfrac{33}{4}t)}
\] Then the approximate solution by Algorithm \ref{alg4} $\wh{x}_{m^{(a)}_k}^k$ at the end of the $k$th stage  of the asymptotic phase
satisfies, with probability $\geq 1-4(\overline{K}_1 +k)e^{-t}$, $\|\wh{x}_{m^{(a)}_k}^k-x_*\|\leq r_k$, implying that
\be \|\wh{x}_{m^{(a)}_k}^k-x_*\|\lesssim  \left(\frac{\sigma_*^2\psi^{2\beta}\left( \sfrac{s}{\lambda}\right)^{{\beta}}\chi \Theta\left(\Theta + t \right) }{\mu^2 N_k}\right)^{\frac{1}{2(\beta - 1) }}, \ee{asymp-phase-batch}
where $N_k = \sum_{i=1}^k m^{(a)}_i \ell_i$ is the total count of oracle calls for $k$ asymptotic stages.
\end{lemma}
\paragraph{Proof.}
Note that proof of Lemma \ref{lem:unifconv2} is very similar to the proof of Lemma \ref{lem:unifconv}. The proof starts similarly as previously except that now we consider the sequence $(r_k)_{k\geq 0}$ and we replace at each stage $\sigma_*^2$ by $\overline{\sigma}^2_{*} = \frac{\chi \sigma_*^2 \Theta}{\ell_k}$, i.e., \eqref{prooflemm4.1-2} becomes 
\[
\|\wh x^k_{m^{(a)}_{k}} - x_*\| \leq \psi \left[(\beta -1) \left(\frac{\sqrt{\sfrac{s}{\lambda}}}{\beta \mu^{\frac{1}{\beta}}}\right)^{\frac{\beta}{\beta -1}}\kappa_{k}^{\frac{1}{\beta - 1}}+\frac{\nu r_{k-1}^2}{m^{(a)}_k \kappa_k}\left(4\Theta + 60t\right) +\frac{r_{k-1}}{m^{(a)}_k} + \frac{\chi\sigma_*^2\Theta}{\kappa_k \ell_k\nu}\left(\frac{7}{4} + \frac{6t}{m^{(a)}_k}\right) \right],
\]
We choose the parameters $\kappa_k$ and $m^{(a)}_k$ the same way, except that now, after having chosen $\kappa_k$ and plugged its value in the previous relationship, $m^{(a)}_k$ is chosen to bound each of the appearing first two terms by $\frac{r_{k-1}}{8}$, this choice still implies $\frac{6t}{m^{(a)}_{k}} \leq \frac{1}{4}$ and it results in 
\[
\|\wh x^k_{m^{(a)}_{k}} - x_*\| \leq \frac{r_{k-1}}{4} + \frac{2 \psi \chi\sigma_*^2\Theta}{\kappa_k \ell_k\nu}.
\]
Then we choose $\ell_k$ in order to bound the last term by $\frac{r_{k-1}}{4}$, this finally results in 
\begin{align}
\|\wh x^k_{m^{(a)}_{k}} - x_*\| \leq \frac{r_k}{2} = 2^{-k} r_0.\label{prooflemm4.2-1}
\end{align}
Now let us express the total count of oracle call after $k$ stages of asymptotic stage.
\begin{align*}
N_k &= \sum_{i=1}^k m^{(a)}_i \ell_i = C_0 \frac{\chi \Theta(\Theta +t)s\psi^2\nu^{\frac{2(\beta - 1)}{\beta}} \sigma_*^{\frac{2(2-\beta)}{\beta}} }{\lambda\mu^{\frac{2}{\beta}}}\sum_{i=1}^{k} \\
& = C_1 \frac{\chi \Theta(\Theta +t)s\psi^2\nu^{\frac{2(\beta - 1)}{\beta}} \sigma_*^{\frac{2(2-\beta)}{\beta}} }{\lambda\mu^{\frac{2}{\beta}}}2^{2(\beta - 1)k}.
\end{align*}
By inverting the last inequality, it is possible to express $2^{-k}$ as a function of $N_k$ up to an absolute constant and result \eqref{asymp-phase-batch} follows after plugging this value and the value of $r_0$ within result \eqref{prooflemm4.2-1}
\qed
\begin{theorem}\label{thm:unifconv}
Assume that the total sample budget satisfies $N \geq m^{(p)}_1$, so that at least one stage of the preliminary phase of Algorithm \ref{alg4} is completed, then for $ t\gtrsim \sqrt{\ln N}$, the corresponding solution $\widehat{x}^{(b)}_N$ of the minibatch Algorithm \ref{alg4} satisfies with  probability at least $ 1 - C(\overline{K}_1 + \ov{K}_2)e^{-t}$
\[
    \|\widehat{x}^{(b)}_N - x_*\| \lesssim \left(\frac{\nu (\Theta + t ) (\psi \sqrt{\sfrac{s}{\lambda}})^{\beta}}{\mu N}\right)^{\frac{1}{\beta - 2}}+ \left(\frac{\sigma_*^2\psi^{2\beta}\left( \sfrac{s}{\lambda}\right)^{{\beta}}\chi \Theta\left(\Theta + t \right) }{\mu^2 N}\right)^{\frac{1}{2(\beta - 1) }}.
\]
where $\ov{K}_2 = \max_{k}\left\{ \sum_{i}^{k} m^{(a)}_i \ell_i \leq N - \sum_{i}^{\ov K_1} m^{(p)}_i\right\}$ is the count for the number of stages of the asymptotic phase of the minibatch algorithm.
\end{theorem}
\paragraph{Proof.}
Let assume that the ``total observation budget'' $N$ is such that only the preliminary phase of the procedure is implemented.
This is the case when either $\sum_{i=1}^{\ov K_1}m^{(p)}_i\geq N$, or $\sum_{i=1}^{\ov K_1}m^{(p)}_i< N$ and $\sum_{i=1}^{\ov K_1}m^{(p)}_i + m^{(a)}_1 \ell_1> N$.
The output $\wh{x}_N $ of the algorithm is then the last update of the preliminary phase, and by Lemma \ref{lem:unifconv} it satisfies 
 $\|\wh{x}_N-x_*\|\leq R_k \leq2^{-k + 1}R$
 where $k$ is the count of completed stages.
In this case we have that 
\[
 N \leq C_0 \sum_{i=1}^{k}m^{(p)}_i = C_1 (\psi \sqrt{\sfrac{s}{\lambda}})^{\beta}\nu \mu^{-1}(\Theta + t)\sum_{i= 1}^{k} {R^{-(\beta - 2)}_{i-1}}.
\]
Recall that we have $\forall k,  2^{-k}R \leq R_k$, this together with last inequality leads us to 
\[
 N \leq C_2 (\psi \sqrt{\sfrac{s}{\lambda}})^{\beta}\nu \mu^{-1}(\Theta + t) 2^{k(\beta - 2)} R^{-(\beta-2) }.
\]
We can then show that 
\[
 2^{-k + 1} \leq \frac{C_3}{R} \left(\frac{\nu (\Theta + t ) (\psi \sqrt{\sfrac{s}{\lambda}})^{\beta}}{\mu N}\right)^{\frac{1}{\beta - 2}}.
\]
Finally, we have shown that with probability at least $1 - 4e^{-t}$

\be
\|\wh{x}_N-x_*\|\lesssim \left(\frac{\nu (\Theta + t ) (\psi \sqrt{\sfrac{s}{\lambda}})^{\beta}}{\mu N}\right)^{\frac{1}{\beta - 2}}.
\ee{pbo} 
On the other hand, when $\sum_{i=1}^{\ov K_1}m^{(p)}_i< N<\sum_{i=1}^{\ov K_1}m^{(p)}_i + m^{(a)}_1 \ell_1$, by using the of $m^{(a)}_1$ and $\ell_1$, one has $N\leq C\sum_{i=1}^{\ov K_1}m^{(p)}_i$, so that bound
\rf{pbo} still holds in this case. Here, $C, C_0, C_1, C_2,$ and $C_3$ are absolute constants.

Now, consider the case where at least one asymptotic stage has been completed.
When $\sum_{i=1}^{\ov K_1}m^{(p)}_i>\frac{N}{2}$ we still have $N\leq C \sum_{i=1}^{\ov K_1}m^{(p)}_i$, so that the bound \rf{pbo} holds for the approximate solution $\wh{x}^{(b)}_N$ at the end of the asymptotic stage. Otherwise, the number of oracle calls $N_k$ of asymptotic stages satisfies $N_k\geq N/2$, and by \rf{asymp-phase-batch} this implies that with probability $\geq 1-4(\overline{K}_1+\overline{K}_2)e^{-t}$,
 \[
 \|\wh{x}^{(b)}_N-x_*\|\lesssim \left(\frac{\sigma_*^2\psi^{2\beta}\left( \sfrac{s}{\lambda}\right)^{{\beta}}\chi \Theta\left(\Theta + t \right) }{\mu^2 N}\right)^{\frac{1}{2(\beta - 1) }},
 \]
To summarize, in both cases, the bound of Theorem \ref{thm:reli} holds with probability at least $1-4(\overline{K}_1+\overline{K}_2)e^{-t}$.
%The proof of the accuracy bound for the ``standard'' solution $\wh x_N$ is completely analogous, making use of the bound \rf{asymp-phase-nobatch} of Lemma \ref{ya2222}  instead of \rf{asymp-phase-batch}.
\qed
\\
We can then give the related algorithm.

\begin{algorithm}[H]
\caption{CSMD-SR}\label{alg4}
\textbf{Initialization :} Initial point $x_0\in X$, step-size $\gamma = (4\nu)^{-1}$, initial radius $R_0$, confidence level $t$, total budget $N$.
\\ Set $m^{(p)}_1\asymp{(\delta\sqrt{s\over\lambda} )^{\beta}{\nu\over\mu}{(\Theta+t)\over R_{0}^{\beta-2}}}$, $\overline{K}_1 \asymp \ln\left(\frac{R_0^{\beta}\nu \mu}{  \sigma^2_* \delta^{\beta}(s/\lambda)^{\beta/2}}\right)\wedge {N\over m_1}$, $L =1$
\begin{algorithmic}[1]
\State \textbf{if} 
\State\quad $R_0 \gtrsim \delta\sqrt{ \sfrac{s}{\lambda}} (\sfrac{\sigma_*^2}{ \nu \mu})^{\frac{1}{\beta}}$ continue with preliminary stage,
\State \textbf{else} proceed directly with asymptotic phase
\State \textbf{endif}
\For{\textbf{stage} $k=1,\dots, \overline{K}_1 $}\Comment{\underline{Preliminary Phase}}
\State Set $\kappa_k  \asymp {R_{k-1}^{\beta - 1} \mu }{\psi^{-(\beta - 1)} \sqrt{\sfrac{\lambda}{s}}^{\beta}}$
\State Compute approximate solution $\widehat{x}^k_{m^{(p)}_k}= $ CSMD($x_0, \gamma, \kappa_k, R_{k-1}, m^{(p)}_k, L$) at stage $k$
\State Reset the prox-center $x_0 = \widehat{x}^k_{m_k}$
\State Set $R_k = R_{k-1}/2$
\State Set $m^{(p)}_{k+1} = 2^{\beta - 2} m^{(p)}_k$

\EndFor
\State Set $\widehat{x}_N = \widehat{x}_{m^{(p)}_{\overline{K}_1}}^{\overline{K}_1}$, $B = N - \sum_{i=1}^{\overline{K}_1} m^{(p)}_i $.
\State Set $r_0 = R_{\overline{K}_1}$
\State Set $\ell_1 \asymp \chi \Theta$
\State Set $m^{(a)}_1 \asymp r_0 \delta\sqrt{\sfrac{s}{\lambda}}\left(\Theta + t \right)\left(\sfrac{\nu}{\sigma_*^{2}}\right)^{\frac{\beta - 1}{\beta}} \mu^{-\frac{1}{\beta}} $
\State\textbf{if} {$m_1 >B$} \textbf{output :} $\widehat{x}_N$ and \textbf{return}; \textbf{endif}\Comment{\underline{Asymptotic Phase}}
\State Set $k = 1$
\While{$m^{(a)}_k \ell_k \leq B$}
\State Set $\kappa_k \asymp 2^{-k({\beta - 1})}\mu^{\frac{1}{\beta}}\sqrt{\sfrac{\lambda}{s}}  \left(\sfrac{\sigma_*^{2}}{\nu}\right)^{\frac{\beta - 1}{\beta}}$.
\State Compute approximate solution $\widehat{x}^k_{m^{(a)}_k}= $ CSMD($x_0, \gamma , \kappa_k, r_{k-1}, m^{(a)}_k, L = \ell_k$) at stage $k$
\State Reset the prox-center $x_0  = \widehat{x}^k_{m^{(a)}_k}$
\State Set $B = B - \ell_k m^{(a)}_k$, $k=k+1$, $r_k = r_{k-1}/2$, $m^{(a)}_k \asymp 2^{(\beta - 2)k} \left(\Theta + t \right)\left(\sfrac{\nu}{\sigma_*^{2}}\right)^{\frac{\beta - 1}{\beta}} \mu^{\frac{2}{\beta}} \sqrt{\sfrac{\lambda}{s}}$.
\State Set $ \ell_k \asymp 2^{\beta k} \ell_1$.
\EndWhile
\end{algorithmic}
\textbf{output :} $\widehat{x}_N = \widehat{x}^{k-1}_{m^{(a)}_{k-1}}$
\end{algorithm}

\newpage

